Unsupervised Neural Text Simplification

The paper presents a first attempt towards unsupervised neural text simplification that relies only on unlabeled text corpora. The core framework is composed of a shared encoder and a pair of attentional-decoders and gains knowledge of simplification through discrimination based-losses and denoising. The framework is trained using unlabeled text collected from en-Wikipedia dump. Our analysis (both quantitative and qualitative involving human evaluators) on a public test data shows that the proposed model can perform text-simplification at both lexical and syntactic levels, competitive to existing supervised methods. Addition of a few labelled pairs also improves the performance further.

==> 4_system.tex <==
Our model has a single shared encoder \(E\) and two decoders \(G_s\), \(G_d\). Encoder \(E\) and decoders \(G_s\), \(G_d\) follow standard attentional encoder-decoder model proposed by \newcite{bahdanau2014neural}. Encoder (\(E\)) is a two layered bi-directional RNN, whereas decoders(\(G_s\),\(G_d\)) are standard two layered RNNs. \(E\), \(G_s\) and \(G_d\) are built on GRU cells. Pipelines \(E-G_s\), \(E-G_d\) aim to simplify and complicate the input sentence. Here encoder is shared between both domains (simple, complex or difficult) and is aimed at creating domain invariant hidden representations as shown in Figure \ref{figs:workflow}. Decoders are then used to transfer these representations to their own domains respectively.

Our architecture is similar to NMT model in \newcite{artetxe2018iclr} except, we don't use different embeddings for simple and difficult domains, as they share a single language. All embedding layers in our system are initialized with \emph{dict2vec} embeddings; \emph{dict2vec} is known to capture lexico-semantic relationships such as synonymy better \cite{tissier2017dict2vec}.  We train \textit{dict2vec} embedding of 300 dimensions using en-wikipedia dump using similar settings as \newcite{tissier2017dict2vec}. During training, these embeddings at the encoder are frozen, whereas embeddings at decoder are allowed to be updated.
    
Our training procedure tunes the pipelines so that sentence from {$\boldsymbol{\mathcal{D}}$} domain (domain of difficult sentences) will be simplified when passed through simplifying pipeline \(E-G_s\) and be unchanged when passed through complicating pipeline \(E-G_d\). Sentences from {$\boldsymbol{\mathcal{S}}$} are treated similarly. An ideal simplifying decoder \(G_s\) attends to important content in source, whereas, ideal complicating decoder \(G_d\) attends to the source content in a redundant fashion giving longer attended sequences and thus longer and comprehensive decodings
% \textcolor{red}{What do you mean by redundant fashion? Explain better.}. 
To model this behaviour, discriminators \(D_s\) and \(D_d\) are employed to identify whether the attended vectors \(\boldsymbol{av}\) contain signals related to simple, complex linguistic forms respectively. \(D_s\) is used for helping \(G_s\) to extract simple contents and \(D_d\) for complicating decoder \(G_d\). Here the discriminators extract features and classify using multiple convolution layers followed by concatenation, max pooling, fully connected layer and softmax similar to \cite{kim2014convolutional}.

We introduce classifier $C$ which identifies whether attended vectors \(\boldsymbol{av}\) belong to simple/complex domain. This classifier $C$ is intended to give $G_s$ and $G_d$ additional information about simple domain other than what is provided by discriminators $D_s$ and $D_d$. All discriminators $D_s$, $D_d$ and classifier $C$ share the parameters except the fully connected layer at the end.




==> 8_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In Figure \ref{fig:analysis} we show that during training UnsupNTS-classf-disc baseline touches the 2-4 content reduction band several times during the training than other baselines. The generated simplifications during these times have different simplification schemes. This is because the model is oscillating between low-content reduction to high-content reduction states during training thus making it explore various simplifying alignments of words as well as different ways to conduct content-reduction. Table 2 shows a few examples that make our case. This oscillation cannot occur for long in supervised baselines due to limited data, but the unsupervised dataset we designed has enough examples for the model to explore various ways to simplify a sentence. This observation is consistent with the fact that a sentence can have multiple simplifications, thus inspiring a possibility of controlled simplification framework in which rate of simplification can be controlled by a control variate passed as input.

% TODO: longer sentences causing more content reduction than smaller ones.
The algorithm \ref{algo:algo1} designed is such that sentences from simple domain are auto-encoded by simplifying pipeline and sentences from difficult domain are constrained to be simplified. Table \ref{tab:gens} shows predictions for  4 source sentences for different models of UnsupNTS-classf-adv baseline. The first 2 source sentences change drastically reflecting the effect of classifier and adversarial losses, whereas the last two source sentences don't change much when passed through simplifying pipeline because they are nearer to simple domain, . 
% The simplifications of first 2 source sentences in Table \ref{tab:gens} by different models for a single sentence shows diverse simplification schemes, one reducing content more than the other.

% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}


==> central.tex <==
\section{Central Idea}
\label{sec:central}
We propose a neural sequence to sequence architecture equipped with attention mechanism which is guided by an adversarial loss, as a result the decoder will attend to only relevant parts of the sentence and ignore the rest while decoding. We also use \textit{denoising} and on-fly \textit{backtranslation} to aid the model by taking advantage of dual nature of the simplification problem. Our training procedure is targeted such that lexical simplification, syntactic simplification and especially content reduction can be performed by the model during inference. We also solve the auto encoding problem faced by NTS models by introducing a mild classifier loss which constrains the model not to attend the source like an autoencoder does. This way our training process becomes sustainable for longer time without reaching an auto encoding state.

TODO: benefits introduced by our training procedure.





==> data-stats.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Category} & \textbf{FK-limits} & \textbf{avg sentence length} & \textbf{no. of sentences} \\ \hline
simple-dataset & 75.2-75.54 & 18.23 & 0.72 million \\ \hline
complex-dataset & 6.85-8.54 & 35.03 & 0.72 million \\ \hline
\end{tabular}
\end{table}
